Learning to Compose Domain-Specific Transformations for Data Augmentation

Data augmentation is a ubiquitous technique for increasing the size of labeled training sets by leveraging task-specific data transformations that preserve class labels. While it is often easy for domain experts to specify individual transformations, constructing and tuning the more sophisticated compositions typically needed to achieve state-of-the-art results is a time-consuming manual task in practice. We propose a method for automating this process by learning a generative sequence model over user-specified transformation functions using a generative adversarial approach. Our method can make use of arbitrary, non-deterministic transformation functions, is robust to misspecified user input, and is trained on unlabeled data. The learned transformation model can then be used to perform data augmentation for any end discriminative model. In our experiments, we show the efficacy of our approach on both image and text datasets, achieving improvements of 4.0 accuracy points on CIFAR-10, 1.4 F1 points on the ACE relation extraction task, and 3.4 accuracy points when using domain-specific transformation operations on a medical imaging dataset as compared to standard heuristic augmentation approaches.

==> tanda_notes.tex <==
\section{General things to mention}
\begin{itemize}
    \item Should mention that the generator is 400x (or more) smaller (by parameter count) than the discriminator--easier to learn when we start with known set of transformations!
\end{itemize}


\section{Notes: Theory Ideas}
\begin{itemize}
    \item Notes from chat with CR:
    \begin{itemize}
        \item Need to argue that they don't commute- this is motivation for sequence
        \item Need to argue / point to that if you have a set of small TFs (semi-group that's locally linear) they can form a kernel
        \item Make assumption that the space of images is path-connected \textit{within classes}
        \item Make t-SNE plot of MNIST with random augmentations
        \item If you can't argue X is right choice, argue you're robust to choice of X
    \end{itemize}

    \item Viewing the TFs as defining a kernel
    \begin{itemize}
        \item Interesting that here we are using a kernel to bootstrap a DL model;
        whereas usually it's the other way around...
    \end{itemize}
    \item Can we say something about \textit{robustness w.r.t. a TF}?
    \begin{itemize}
        \item How is ``robustness w.r.t. a TF defined'' in our context?
        \item If we apply a single TF, can we provide guarantees on the robustness
        of the end model to this TF?
        \item What about if TF is applied with many other TFs?
    \end{itemize}
    \item What about avoiding ``cluster catastrophe'' setup:
    \begin{itemize}
        \item MF: Should be able to learn that certain single TFs are catastrophic
        \item MC: Should be able to learn that certain $k$-sequences are catastrophic
        \item LSTM: Should be able to learn that certain $k$\textit{sets} are catastrophic
    \end{itemize}
    \item Another toy model: Imagine that for each dimension $i$, you have $m_i$ TFs that are random vectors in each dimension.  If you randomly sample over \textit{all} TFs, you'll get a biased answer; if you sample dimensions, then TFs, better...
    \item Conception of two toy models:
    \begin{itemize}
        \item Counting only: Maintain as state a vector representation to ``count'' how many of each TF has been applied
        \item Counting + order: Maintain that state, plus also the order of TFs applied
    \end{itemize}
    \item Simple example: apply fourier transform, then some TFs are only applicable to fourier space!
\end{itemize}

